Searching for Gravitational-Wave Bursts with LIGO

We present recent results from searches by the LIGO Science Collaboration for bursts of gravitational-wave radiation, as well as the status of other ongoing searches. These include directed searches for bursts associated with observed sources (gamma-ray bursts, soft gamma repeaters) and untriggered searches for bursts from unknown sources. We also present the status of some newer investigations, such as coherent network methods. We show methods for interpreting our search results in terms of astrophysical source distributions that improve their accessibility to the wider community.

==> README <==
README file for GR-QC submission

Files:
   README        - this file
   moriond.tex   - LaTeX file of paper
   moriond.sty   - style file for Moriond conference proceeedings
   S1S2S4results-SG20Q8d9.eps - Figure 1
   galpopeff.eps  - Figure 2
   ratestrength.eps - Figure 3  

Title: Searching for Gravitational-Wave Bursts with LIGO

Author: K. A. Thorne, for the LIGO Scientific Collaboration (LSC)

Address: Center for Gravitational Wave Physics \\ Institute for  
Gravitational Physics and Geometry \\ Pennsylvania State University\\
University Park, PA 16802 United States}

Abstract
We present recent results from searches by the LIGO Science
Collaboration for bursts of gravitational-wave radiation, as well as
the status of other ongoing searches.
These include directed searches for bursts associated with observed  
sources (gamma-ray bursts, soft gamma repeaters) and untriggered  
searches for bursts from unknown sources. We also present the status  
of some newer investigations, such as coherent network methods.
We show methods for interpreting our search results in terms of  
astrophysical source distributions that improve their accessibility  
to the wider community.

Submitted to Conference Proceedings of the 
Recontres de Moriond, Gravitational Waves and Experimental Gravity 
March 11-18, 2007

